Bounded Quantifier Instantiation for Checking Inductive Invariants

We consider the problem of checking whether a proposed invariant $\varphi$ expressed in first-order logic with quantifier alternation is inductive, i.e. preserved by a piece of code. While the problem is undecidable, modern SMT solvers can sometimes solve it automatically. However, they employ powerful quantifier instantiation methods that may diverge, especially when $\varphi$ is not preserved. A notable difficulty arises due to counterexamples of infinite size. This paper studies Bounded-Horizon instantiation, a natural method for guaranteeing the termination of SMT solvers. The method bounds the depth of terms used in the quantifier instantiation process. We show that this method is surprisingly powerful for checking quantified invariants in uninterpreted domains. Furthermore, by producing partial models it can help the user diagnose the case when $\varphi$ is not inductive, especially when the underlying reason is the existence of infinite counterexamples. Our main technical result is that Bounded-Horizon is at least as powerful as instrumentation, which is a manual method to guarantee convergence of the solver by modifying the program so that it admits a purely universal invariant. We show that with a bound of 1 we can simulate a natural class of instrumentations, without the need to modify the code and in a fully automatic way. We also report on a prototype implementation on top of Z3, which we used to verify several examples by Bounded-Horizon of bound 1.

==> existence_low_bound_invariants.tex <==
\def\instformula#1{\varphi^{#1}}
%\def\witnessvar#1#2{y_{#2}^{#1}}
\def\witnessvar#1#2{y_{f_{#2}(#1)}}
\def\witnessvarset{\mathcal{Y}}
\def\skolwitness#1{F_{#1}}

\section{Existence of Low-Bound Invariants}
In this section we investiage the existence of inductive invariants provable using a low bound.

Let $\delta$ be transition relation and $I \in \AE$ an inductive invariant for $\delta$.
As \Cref{bh:exists-k} shows, there exists $k \in \Nat$ s.t.\ $I$ is provably inductive for $\delta$ with Bounded-Horizon of bound $k$.
We will construct $I^{*}$ an inductive invariant for $\delta$ equivalent to $I$, with the property that it is provable with Bounded-Horizon of bound just $2$.
In essence $I^{*}$ will encode the instantiations required for proving that $I$ is inductive in an incremental fashion, allowing bound $2$ reasoning to simulate the original bound $k$ proof.

$I^{*}$ that we construct in this paper is a 1-alternation sentence, although the invariant we begin with, $I$, is $\AE$.
It remains an open questions whether a similar result can be obtained for $I^{*}$ that is $\AE$ as well, or $I^{*}$ 1-alternation with the weaker assumption that $I$ is 1-alternation.
Another open question is whether such an invariant can be constructed to be provable using Bounded-Horizon of bound 1, or perhaps there exist transition relations for which a $\AE$ or 1-alternation invariant exists, but not one that is provable by bound 1.

Throughout this section we denote the invariant by
\begin{equation}
I = \forall x_1, \ldots, x_n. \ \exists y_1, \ldots y_m. \ \varphi(x_1, \ldots, x_n, y_1, \ldots, y_m)
\end{equation}
where $\varphi \in \QF$.

\paragraph{Encoding higher bounds.}
We define $I_r$ the expansion of $I$ to bound $r$ (for $r \in \Nat$) in the following way:
Consider the Skolemization of $I$, $\sk{I}$, that introduces Skolem functions $f_1, \ldots, f_m$ of arity $n$.
We encode instantiations of the universal quantifiers with $\bhterms{r}$ terms in the following way:
For $\vec{t} = t_1, \ldots, t_n \in \bhterms{r}$ and $1 \leq j \leq m$ we define a fresh variable $\witnessvar{\vec{t}}{j}$. Let this set of variables be $\witnessvarset$.
Intuitively, each term is generated from its subterms by an application of the Skolem function that we would like to encode using an existential quantifier.
Techincally, for every $t_i$ we have a corrseponding generating variable $z_i$:
if $t_i$ is a constant, take $z_i = x_i$.
Otherwise $t_i = f_j(\vec{\tilde{t}})$ for some function $f_j$ and term $\vec{t}$.
In this case let $z_i = \witnessvar{\vec{\tilde{t}}}{j}$.
The connection between $\vec{t}$ and the terms it generates is expressed by the formula
\begin{equation}
\instformula{\vec{t}} = \varphi(z_1, \ldots, z_n, \witnessvar{\vec{t}}{1}, \ldots, \witnessvar{\vec{t}}{m}).
\end{equation}
\yotam{Note: redundancy because different constants do not make a difference, they are all mapped to $x_i$}

We can now define the expanded invariant.
\begin{definition}
\begin{equation}
I_{r} =
\forall x_1, \ldots, x_n. \
\mathop{\exists}_{\witnessvar{\vec{t}}{j} \in \witnessvarset}{\witnessvar{\vec{t}}{j}}
\bigwedge_{\vec{t} \in \bhterms{r}}{
	\instformula{\vec{t}}
}
\end{equation}
where the conjunction is over tuples of terms $\vec{t}$ that generate an instantiation of bound at most $r$, meaning $\instdepth{\sk{I}}{\vec{t}} \leq r$.
\end{definition}

\begin{lemma}
\label{lem:existence_expanded_equiv}
$I_r$ is logically equivalent to $I$ for every $r \in \Nat$.
\end{lemma}

\begin{lemma}
\label{lem:existence_unsat_k_1_by_1}
$I_k \land \delta \land \neg I'_1$ is unsatisfiable by bound 1 instantiations.
\end{lemma}
\begin{proof}
This is a corollary of $I \land \delta \land \neg I'$ being unsatisfiable by bound $k$ instantiations.
Assume for the sake of contradiction that $\A$ is a structure satisfying bound $1$ instantiations of $\sk{(I_k)} \land \sk{\delta} \land \sk{(\neg I'_1)}$.
Without loss of generality assume that $\A$ is a Herbrand structure\footnote{
	A Herbrand structure assumes that the underlying logic is without equality. For FOL with equality, first add the theory of equality for the vocabulary $\Sigma$ in conjunction to the formula and continue by checking satisfiability in FOL without equality. Note that this is possible because the theory of equality is universal.
}.
We will reach a contradiction by constructing $\A'$, a model of the bound $k$ instantiations of $\sk{I} \land \sk{\delta} \land \sk{(\neg I')}$.

$\A'$ has the same domain as $\A$ and the same interperation of constants and relations of $\Sigma$.
We also need to provide an interepretation for the additional Skolem constants and functions in $\sk{I} \land \sk{\delta} \land \sk{(\neg I')}$.
Denote these Skolem functions by $g_1, \ldots, g_m$, each is of arity $n$.
The interpretation makes sure that \TODO{continue}

\end{proof}

\paragraph{The low-bound invariant.}
\begin{definition}
\begin{equation}
I^{*} = I_1 \land (I_1 \rightarrow I_2) \land \ldots \land (I_{k-1} \rightarrow I_k)
\end{equation}
\end{definition}

\begin{lemma}
$I^{*}$ is logically equivalent to $I$.
\end{lemma}
\begin{proof}
Follows directly from \Cref{lem:existence_expanded_equiv}.
\end{proof}

\begin{corollary}
$I^{*} \land \delta \land \neg I'_1$ is unsatisfiable by bound 1 instantiations.
\end{corollary}
\begin{proof}
$I^{*} \land \delta \land \neg I'_1$ in NNF reads $I_1 \land (\neg I_1 \lor I_2) \land \ldots (\neg I_{k-1} \lor I_k) \land \delta \land \neg I'_1$, we will refer to it as $\xi$.
Intuitively, instantiating the universal quantifiers of $I_1$ with the Skolem constants that are introduced by $\neg I_1$ ``implies" that $I_2$ must hold.
Continuing in this fashion, such simple instantiations establish that $I_k$ must hold, and \Cref{lem:existence_unsat_k_1_by_1} already shows that $I_k \land \delta \land \neg I'_1$ is unsatisfiable by bound 1 instantiations.

More formally, from \Cref{lem:existence_unsat_k_1_by_1} we have a set of bound 1 instantiations of $I_k \land \delta \land \neg I'_1$ that is unsatisfiable.
Augment each instantiation by an instantiation of the rest of the universal quantifiers in $\sk{\xi}$ by instantiating every universal quantifier in $\sk{(I_r)}$, for $1 \leq r \leq k-1$, by the corrseponding Skolem constant from $\sk{(\neg I_r)}$.
The resulting set of instantiations of $\xi$ is also of bound 1 and unsatisfiable.
\end{proof}

\paragraph{Provability by bound 2.}
\begin{lemma}
$I_r \land \neg I_{r+1}$ is unsatisfiable by bound 2 instantiations for every $r \in \Nat$.
\end{lemma}
\begin{proof}
Intuitively, $I_{r+1}$ encodes one additional level of instantiations compared to $I_r$, but instantiating the universal quantifiers of $\sk{(I_r)}$ with $\bhterms{0}$ and $\bhterms{1}$ suffices to deduce the instantiations of $I_{r+1}$ from those of $I_r$.
$\sk{(\neg I_{r+1})}$ means that for some constants $d_1, \ldots, d_n$ none of the bound $r+1$ instantiations hold, and we can refute that by generating these instantiations with depth 1 and 2 instantiations of $\sk{(I_r)}$.

Formally, assume for the sake of contradiction that there is a structure $\A$ satisfying all bound 2 instantiations of $\sk{(I_r)} \land \sk{(\neg I_{r+1})}$.
Let $\vec{d} = d_1, \ldots, d_n$ be the Skolem constants introduced by $\sk{(\neg I_{r+1})}$.
The Skolemization of $I_r$ introduces Skolem functions $\skolwitness{f_j(\vec{t})}$ (for every $\vec{t}$ such that $\instdepth{\sk{I}}{\vec{t}} \leq r$ and $1 \leq j \leq m$).

Consider the instantiation of the universal quantifiers in $\sk{(\neg I_{r+1})}$ in the following way:
Let $\witnessvar{\vec{t}}{j}$ be a universally quantified variable in $\sk{(\neg I_{r+1})}$.
By definition this means that $\instdepth{\sk{I}}{\vec{t}} \leq r + 1$.
There exist $\vec{s} = s_1, \ldots, s_n \in \bhterms{r}$ s.t.\ $\instdepth{\sk{I}}{\vec{s}} \leq r$

Thus, in particular, there is a valuation $v$ in $\A$ such that
\begin{equation}
  \A, v \models \varphi(d_1, \ldots, d_n,
		    \skolwitness{f_1(\vec{t})}(\vec{d}), \ldots, \skolwitness{f_m(\vec{t})}(\vec{d}))
\end{equation}
%\begin{equation}
%  \A, v \models \varphi(d_1, \ldots, d_n,
%		    \skolwitness{f_1(\vec{t})}(\vec{d}), \ldots, \skolwitness{f_m(\vec{t})}(\vec{d}))
%\end{equation}
%for every $\vec{t} \in \bhterms{r}$ s.t.\ $\instdepth{\sk{(I_r)}}{\vec{t}} \leq r$,
%and also
%\begin{equation}
%  \A, v \models \varphi(f_{j_1}(\vec{t_1}), \ldots, f_{j_n}(\vec{t_n}),
%		    \witnessvar{\vec{t}}{1}, \ldots, \witnessvar{\vec{t}}{m})
%\end{equation}
%\begin{equation}
%  \A, v \models \varphi(t_1, \ldots, t_n,
%		    \witnessvar{\vec{t}}{1}, \ldots, \witnessvar{\vec{t}}{m})
%\end{equation}
%for every $t_1, \ldots, t_n \in \bhterms{2}$ s.t.\ $\instdepth{\sk{(I_r)}}{t_1, \ldots, t_n} \leq 2$.
%\begin{equation}
%  \A, v \models \varphi(s_1, \ldots, s_n,
%		    \skolwitness{f_1(\vec{t})}(\vec{s}), \ldots, \skolwitness{f_m(\vec{t})}(\vec{s}))
%\end{equation}
%for every $\vec{s} \in \bhterms{2}$ s.t.\ $\instdepth{\sk{(I_r)}}{\vec{s}} \leq 2$.

TODO we probably need the notion of the template that plug in the variables $d_1, \ldots, d_n$?
\end{proof}

\begin{corollary}
$I^{*} \land \delta \land \neg I^{*}$ is unsatisfiable by bound 2 instantiations.
\end{corollary}
\begin{proof}
\end{proof}
And the theorem follows:
\begin{theorem}
Let $\delta$ be a transition relation. If there exists a $\AE$ inductive invariant for $\delta$ then there exists a $\ONEALT$ inductive invariant for $\delta$ provable by Bounded-Horizon of bound 2.
\end{theorem}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> fol-syntax.tex <==
\begin{figure}
\[
\arraycolsep=10pt
\begin{array}{||cclr||}
\hhline{|t:====:t|}
\nonterm{t} & ::= & & \mbox{terms}
\\
& | & x & \mbox{logical variable}~x
\\
& | & c & \mbox{constant symbol}~c
\\
& | & f \left(\nonterm{t},\ldots,\nonterm{t} \right) & \mbox{application of function}~f
\\
&&&
\\
\nonterm{\varphi} & ::= & & \mbox{formulas}
\\
%% & | & \true & \mbox{literal true}
%% \\
%% & | & \false & \mbox{literal false}
%% \\
& | & r \left(\nonterm{t},\ldots,\nonterm{t} \right) & \mbox{membership in relation}~r
\\
& | & \nonterm{t} = \nonterm{t}  & \mbox{equality between terms}
\\
& | & \nonterm{\varphi} \land \nonterm{\varphi} & \mbox{conjunction}
\\
& | & \nonterm{\varphi}  \lor \nonterm{\varphi} & \mbox{disjunction}
\\
& | & \nonterm{\varphi}  \to \nonterm{\varphi} & \mbox{implication}
\\
& | & \nonterm{\varphi}  \leftrightarrow \nonterm{\varphi} & \mbox{bi-implication}
\\
& | & \neg \nonterm{\varphi}  & \mbox{negation}
\\
& | & \forall x. \; \nonterm{\varphi}  & \mbox{universal quantification}
\\
& | & \exists x.\; \nonterm{\varphi}  & \mbox{existential quantification}
\\
\hhline{|b:====:b|}
\end{array}
\]
\caption[Syntax of first-order logic]{\label{fig:fol-syntax}%
Syntax of terms and formulas in first-order logic.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> undecidability-reduce-from-halt.tex <==
\section{Undecidability}
\label{sec:undecidability}
For a universal formula $I \in \forall^*(\Sigma)$, the formula $I \land \delta \land \neg I'$ is in EPR (recall that $\delta$ is specified in EPR). Hence, checking inductiveness amounts to checking unsatisfiability of an EPR formula, and is therefore decidable. The same holds for $I \in AF(\Sigma)$. However, this is no longer true when quantifier alternation is introduced. For example, checking inductiveness of $I \in \forall^* \exists^* (\Sigma)$ amounts to checking unsatisfiability of a formula in a fragment for which satisfiability is undecidable.
In this section we show that in fact checking inductiveness of $\AE$ formulas is undecidable, even when the transition relation is restricted to $\EPR$.
The undecidability of the problem justifies sound but incomplete algorithms for checking inductiveness, one of which is the Bounded-Horizon algorithm (defined in \Cref{sec:bounded-horizon}) which we study in this thesis.

\ultpara{Finite and infinite structures.}
We begin by showing that the problem is undecidable when structures, or program states, are assumed to finite.
This is the intention in most application domains~\cite{DBLP:books/daglib/0095988} (including the examples in \Cref{sec:implementation}), \yotam{Cite also something else?} especially when the program does not involve numerical computations.
However, in this thesis we will mostly concern ourselves with the problem of checking inductiveness when structures may also be infinite.
This is because SMT-based deductive verification relies on proof techniques from standard first-order logic, whose semantics is defined over \emph{general} structures, i.e.\ both finite and infinite.
We thus show an undecidability result for this setting as well.
It is interesting to note that the discrepancy between the intended finiteness of the domain and the proof techniques, that cannot incorporate this assumption, will re-emerge in \Cref{sec:partial-models}.

We refer to \emph{inductiveness over finite structures} when the validity of $I \land \delta \rightarrow I'$ is over finite structures, and
to \emph{inductiveness over general structures}, when it is over both finite and infinite structures.

\section{Proof Scheme}
\label{subsec:undecide-tiling}
The undecidability proofs of this section are by reductions from the halting problem, encoded via tiling.
We briefly recall the definition of a tiling problem and the reduction from the halting problem to tiling, on which we will base the undecidability proofs.
\begin{definition}[\cite{CSL:ImmermanRRSY04}]
\yotam{plagiarize from CSL'04}
A \emph{tiling problem} consists of a finite set of tiles $T$ with designated tiles $T_{\text{start}}, T_{\text{halt}} \in T$, along with horizontal and vertical adjacency relations $H,V \subseteq T \times T$.
A \emph{solution} to a tiling problem is an arrangement of instances of the tiles in a rectangular grid (``board'') such that the tile $T_{\text{start}}$ appears in the top left position, the tile $T_{\text{halt}}$ appears on the board, and adjacency relationships $H,V$ are respected, meaning: if a tile $t_2$ appears immediately to the right of $t_1$ it must hold that $(t_1, t_2) \in H$, and if a tile $t_2$ appears immediately under $t_1$ it must hold that $(t_1, t_2) \in V$.
\end{definition}
Tiling problems are undecidable~\cite{CSL:ImmermanRRSY04,BGG}.
The proof is by a reduction from the halting problem: given a Turing machine we can compute a tiling problem such that the problem has a solution iff the machine halts (on the empty input).
In the reduction, rows represent the tape of the Turing machine, as it evolves over time (computation steps)~\cite{BGG}.
Additionally the tiles encode the location of the head and the current (control) state of the machine.
The horizontal and vertical constraints impose that the successive tiled rows correspond to a correct step of the machine, and correspond to the locality of computation.
We briefly explain how this is done (see~\cite{BGG}\TODO{cite appendix} for further details on the construction):
\begin{itemize}
  \item Locations that are not affected by the head's move use \emph{Alphabet tiles}, which simply represent the letter on the tape. The vertical constraint imposes that the same letter will appear in the next line (either with the same tile or one encoding the same letter but with additional control information).

  \item The tile where the head is located uses \emph{Action tiles}. An Action tile encodes not just the letter on the tape but also the current state. The vertical constraint imposes that the tile below, representing the same tape location in the next configuration (after the step) has the correct letter, according to the transition function of the Turing machine.
  The horizontal constraint uses \emph{Merging tiles} to propagate the change of control state to the new location of the head (either to the left or to the right of the action tile, according to the movement of the head in the transition function of the Turing machine).
  The vertical constraints for Merging tiles make sure that the tile below the tile to the left/right of the current Action tile has an Action tile with the correct new state and with the same letter on the tape.

  \item Special tiles are used for the first line, i.e.\ the initial configuration.
  The tile $T_{\text{start}}$ is supposed to appear in the top-left corner and is a sort of Action tile (representing the first transition of the machine), and it imposes the rest of the first line to encode the empty tape.

  \item For terminating configurations of the Turing machine we use a special tile $T_{\text{halt}}$ as the Action tile. \yotam{Does not appear in the book, but does appear in Neil's def, not with explaining its part in the reduction}
\end{itemize}
\TODO{blank tile?}

\TODO{every partial tiling is a partial run of the TM}

\begin{comment}
A useful feature for our purpose is that placing tiles to encode the run of the Turing machine it can be performed by placing tiles in the rectangle in a very simple order: starting from the top-left position, place the unique tile that fits to the right until and the end of the first line.
Then start with the second line, placing there the unique tile that fits there (to the bottom of the top left position) and continue to tile the row, and so on.
Beyond the end of the line (i.e.\ outside the rectangle) corresponds to untouched tape that therefore remains empty.
\end{comment}
A useful feature, for our purpose, is that placing tiles to encode the run of the Turing machine can be performed by placing tiles in the rectangle in a very simple order:
Start with $T_{\text{start}}$ at the top-left position, place the matching merge tile immediately to its right, and continue to tile the first row with blank letter tiles.
Then move to the next line. Tile according to the vertical constraints, introducing an Action tile where necessary (again, according to the vertical constraints) and a Merge tile immediately before or after the Action tile (according to the horizontal constraints).
Thus, choosing the next tile to place depends only on the tiles immediately to the left, immediately up, and (possibly) up and to the right.
Since the number of tiles is finite the number of choice rules is finite, and so this decision is EPR expressible (it is quantifier-free given successors and predecessors of total orders, which are EPR expressible).
We will use this to describe the computation of the Turing machine as a transition system that places a single tile in each step, which we will specify using EPR.
\yotam{I understood from Neil's email that there's always a unique tile to place so the update code can just choose a valid tile, but I don't understand how it's true for the tiling problems originating from the reduction. Perhaps this is true with some transformation of the tile set?}
\sharon{why? if you take a deterministic TM?}

\ultpara{Scope of the proofs.}
%Given a tiling problem we produce a transition relation with an invariant that is inductive iff there is/isn't a finite tiling (depending on the direction that is enumerable).
Although technically it is also possible to prove the results by a trivial reduction from the satisfiability of $\AE$ formulas (since invariants for the transition relation $\true$ necessarily are either valid or unsatisfiable), we believe that the proofs presented here demonstrate the intuition behind the inherent difficulty of checking inductiveness of $\AE$ formulas in a more profound way.

To further provide intuition, in the proofs we prove the undecidability of a closely related problem, that of checking \emph{inductive invariants for safety of transition systems}.
Given a transition relation $\delta$ (over $\Sigma \uplus \Sigma'$), a sentence $\Init$ (over $\Sigma$) describing the set of initial states and a sentence $\PhiProp$ (over $\Sigma$) describing the safety property, the problem is to check whether $\Init \rightarrow I$ (initiation), $I \land \delta \rightarrow I'$ (consecution), and $I \rightarrow \PhiProp$ (safety) are valid (over finite or general structures).
%We refer to \emph{inductiveness over finite structures} when the validity in question is over finite structures, and \emph{inductiveness over general structures} when it is over both finite and infinite structures.
We will consider this problem when $I \in \AE$, $\Init \in \Univ$, $\PhiProp \in \Univ$.
We will further %restrict the problem to
consider instances where $\Init \rightarrow I$ and $I \rightarrow \PhiProp$ are valid, and it only remains to check whether $I \land \delta \rightarrow I'$ is valid.
\sharon{changed to "under these restrictions"} Under these restrictions, the undecidability of the problem of checking inductive invariants for safety of transition systems implies the undecidability of the problem of checking inductiveness. \yotam{as used elsewhere in this thesis?}
\sharon{I removed it since this means over general structures but the paragraph still talks about both cases. Can add back if you'd like} % as used elsewhere in this thesis.
%We refer to \emph{inductiveness over finite structures} when the validity in question is over finite structures, and \emph{inductiveness over general structures} when it is over both finite and infinite structures.
%The problem of checking inductiveness as we defined in \Cref{sec:preliminaries} can be reduced to this problem by taking $\Init = \PhiProp = \true$.
%This problem can be reduced to the problem of checking inductiveness as we defined in \Cref{sec:preliminaries} by checking inductiveness of the $\AE$ formula $(\Init \lor I) \land \PhiProp$.\footnote{
%	The reduction assumes that $\PhiProp$ is a conjunct in $I$; this holds for the invariants constructed in our proofs, and so they establish undecidability also with this restriction on $I$.
%}
%Thus, the undecidability of the problem of checking inductive invariants for safety of transition systems over general structures implies the undecidability of the problem of checking inductiveness as used elsewhere in this thesis.

\section{Inductiveness Over Finite Structures}
\begin{theorem}
\label{thm:undecidability-finite}
It is undecidable to check given $I \in \AE$ and $\delta \in \EPR$ whether $I$ is inductive for $\delta$ over finite structures.
\end{theorem}

\begin{proof}
The proof is by a reduction from the non-halting problem expressed via tiling to the problem of checking inductive invariants for safety of a transition system (over finite structures) where the initiation and safety requirements are valid.
We think of the transition relation $\delta$ as incrementally placing tiles in a rectangle.

\ultpara{Vocabulary.}
The two dimensions of the rectangle are encoded by two total orders: a horizontal order and a vertical order.
When the order is clear from the context, we use $i-1$ as a shorthand for the predecessor of $i$ in the order, and $0$ as a shorthand for the minimal element of the order.
$\text{max}$ is a constant axiomatized to be the maximal element of the horizontal order. We sometimes refer to the lexicographic order of the vertical and horizontal orders as the \emph{board order}.

The transition system keeps track of the last tile placed on the board by a relation $M(i,j)$ which is true only for the last updated location. Since the placing of tiles occurs in a sequential manner we also call this board location \emph{maximal}, and a location \emph{active} if it comes before the maximal location in the board order.

The state of tiles on the board is represented by a set of relations $\{T_k\}$, one for each tile type, encoding the locations on the board where a tile of type $T_k$ is placed.

\ultpara{Transitions.}
In every step the transition system places the next %(unique)
tile that fits in the next location (encoding the next step of the Turing machine).
A step begins with choosing the next %(unique)
tile type $T_{\text{next}}$ to place in the next location. Placing it on the board is done by an EPR update of the (two-vocabulary) form
\begin{equation}\begin{split}
\label{eqn:undecidability-tile-update}
&\forall i,j. \ M'(i,j) \leftrightarrow \left(\left(j = 0 \land M(i-1, \text{max}\right) \lor \left(j \neq 0 \land M(i,j-1)\right)\right)
\\
&\forall i,j. \ T'_{\text{next}}(i, j) \leftrightarrow \left( T_{\text{next}}(i,j) \lor M'(i,j) \right)
\\
&\forall i,j. \ T'_{k}(i, j) \leftrightarrow T_{k}(i, j) \qquad \forall T_k \neq T_{\text{next}}.
\end{split}\end{equation}
As was mentioned in \Cref{subsec:undecide-tiling}, computing the next tile type, $T_{\text{next}}$, is expressible in $\EPR$ (corresponding to locality of computation).
Thus the EPR formula describing a step of the system consists of a disjunction between choices for $T_{\text{next}}$.
Each of these possible choices is described via a conjunction of a guard that makes sure that it is legal to place  $T_{\text{next}}$ and a corresponding update to the relation that is a conjunction of the formulas in \Cref{eqn:undecidability-tile-update}.
%with guards \sharon{guard makes it sound like implication which would turn the EPR to AE. Perhaps say: guards that are conjoined with the update} to make sure that it is legal to place it, each of these possible choices come with a corresponding update to the relation that is a conjunction of the formulas in \Cref{eqn:undecidability-tile-update}.
\sharon{rephrased. Is it ok?}

\ultpara{Initial state.}
Initially we have a unique tile, $T_{\text{start}}$, placed in the upper-left corner, so $\forall i,j. \ T_{\text{start}}(i,j) \leftrightarrow \left( i=0 \land j=0 \right)$ and $\forall i,j. \ \neg T_k(i,j)$ for every other tile type $T_k$.

\ultpara{Safety property.}
The safety property states that the special tile $T_{\text{halt}}$, corresponding to a halting state of the Turing machine, is not placed in any active location on the board.

\ultpara{Invariant.}
The invariant states that up to the maximal location, encoded by $M(i,j)$, we have a valid partial tiling. We require this by a $\AE$ formula saying that for every tile placed in an active location except for the maximal there is a successor tile, that conforms to the (local) tiling rules.\footnote{
  We specify the requirement in this forward fashion, rather than requiring that every tile has a valid predecessor, in order to reuse this invariant in the proof of \Cref{thm:undecidability-infinite}.
}
%
We also add the safety property to the invariant.

%The invariant further states that the special tile $T_{\text{halt}}$, corrseponding to a halting state of the Turing machine, is not placed in any active location on the board.
%We add this to the invariant as well (thus ensuring that the safety requirement is valid).

%\sharon{explain why initiation is also valid?}

%\sharon{better yet: define safety separately from invariant, before invariant. then in invariant explain that it is also conjoined with the safety, and explain why both initiation and safety are valid}

\ultpara{Reduction argument.}
The invariant holds for the initial state, and trivially implies the safety property.

If the machine halts, a counterexample to induction can be obtained by encoding the last execution step of the machine, that is, placing $T_{\text{halt}}$ on the board in a valid tiling.

\sharon{rewrite the following} \yotam{reprhased}
For the converse, assume that the invariant is not inductive over finite structures, i.e., there exists a finite counterexample to induction, and show that the machine halts. The reasoning is as follows:
A finite state satisfying the invariant induces a valid partial tiling.
Since the transition system always places a tile that respects the horizontal and vertical constraints, it is easy to see that a counterexample to induction must place $T_{\text{halt}}$ on the board, and that this also induces a valid partial tiling in the post-state.
Thus a finite counterexample to induction implies the existence of a valid tiling with $T_{\text{halt}}$ on the board, which encodes a terminating computation of the machine.
%If the machine never halts there cannot be a valid finite partial tiling with $T_{\text{halt}}$ on the board, because it would imply a valid finite run of the machine that ends in a halting configuration.
%Namely \yotam{is it namely?}, a valid finite partial tiling necessarily represents a reachable configuration of the Turing machine. If $T_{\text{halt}}$ is on the board, it implies that a halting configuration is reachable. Therefore $T_{\text{halt}}$ cannot be on the board, and the invariant must be preserved.

Thus the invariant is inductive iff the Turing machine never halts.
\end{proof}

\section{Inductiveness Over General Structures}
\begin{theorem}
\label{thm:undecidability-infinite}
It is undecidable to check given $I \in \AE$ and $\delta \in \EPR$ whether $I$ is inductive for $\delta$ over general (finite and infinite) structures.
\end{theorem}
\begin{proof}
The proof is by a reduction from the halting problem expressed via tiling to the problem of checking inductive invariants for safety of a transition system (over general structures) where the initiation and safety requirements are valid.

First note that the proof of \Cref{thm:undecidability-finite} does not hold when structures may be infinite.
The reason is that an infinite valid partial tiling may not correspond to reachable configuration of the Turing machine, so there may be such an infinite tiling with $T_{\text{halt}}$ even though the Turing machine never halts\footnote{
    One way to construct such a tiling, using a tile in row $\omega$ of the board, is utilized in the proof that follows.
}.

In fact, the reduction in this proof must be in the opposite direction: the invariant should be inductive iff the machine does not terminate, whereas in the proof of \Cref{thm:undecidability-finite} the invariant is inductive iff the machine does terminate. This is because satisfiability is recursively-enumerable over finite structures and co-recursively-enumerable over general structures (due to the existence of proofs), which reflects on checking inductiveness through the satisfiability check of the formula $I \land \delta \land \neg I'$.

We thus want to have a counterexample to induction when the machine never halts, i.e.\ has an infinite run. As before, runs of the machine are encoded via tiling, only that now an infinite structure can encode an infinite run of the machine. (It is not necessary that an infinite tiling represents a valid infinite run of the machine, but every infinite run can be represented by such a structure.)
We would like to ``detect'' this situation.
Our way to do this is by the observation that induction on the number of tiles must hold when the number of tiles is finite (but unbounded), as in \Cref{thm:undecidability-finite}, but does not necessarily hold when there is an infinite number of tiles.
This idea is implemented by a relation $H$ with the invariant that it is preserved under successor of board locations. In an infinite structure this does not imply that $H$ is true for all locations. A flag $f$ is used to express a transition that is aware of $H$ not being globally true.

Technically, we construct a transition relation similar to the one in the proof of \Cref{thm:undecidability-finite}, with some additions, as follows.

\ultpara{Vocabulary.}
We add a relation $H$ over board locations and a Boolean flag (nullary predicate \yotam{unary predicate?} \sharon{nullary?}) $f$.

\ultpara{Transition.}
%In addition, we hold a relation $H$ with the invariant that it is preserved under successor on the board for all active locations, i.e.: If $(i_1,j_1),(i_2,j_2)$ are active locations and $(i_2,j_2)$ is the successor of $(i_1,j_1)$ w.r.t.\ the board order, then if $H$ holds for $(i_1,j_1)$ it must also hold for $(i_2,j_2)$.
To maintain the invariant that $H$ is preserved under successor of active board locations (see below), when we place a new tile, if $H$ holds for the previous maximal element, set $H$ to true for the new maximal element as well.
If $H$ does not hold on the maximal location, turn $f$ to $\false$.
%To maintain this, whenever we place a tile on the board we set $H$ to true for that location. (Initially $H$ is true on the initial location only.)

%We also add a flag $f$ initialized to $\true$.
%When we make a transition, if $H$ does not hold on the maximal location, turn $f$ to $\false$.

\ultpara{Initial state.}
Initially $H$ is true for the initial location only, and $f$ is $\true$.

\ultpara{Safety property.}
The safety property now asserts that $f$ is $\true$.

\ultpara{Invariant.}
As before, the invariant states that the active board represents a valid partial tiling, i.e.\ every active tile except for the maximal one has a valid successor. %In addition, the invariant states that $H$ holds for all elements of the active domain (this is reminiscent of induction).

In addition, the invariant states that $H$ is preserved under successor of active board locations, i.e.: If $(i_1,j_1),(i_2,j_2)$ are active locations and $(i_2,j_2)$ is the successor of $(i_1,j_1)$ w.r.t.\ the board order, then if $H$ holds for $(i_1,j_1)$ it must also hold for $(i_2,j_2)$.
%
We also add the safety property to the invariant.

\ultpara{Reduction argument.}
%If there is an infinite run of the Turing machine we can construct a structure encoding the corresponding tiling.
The invariant holds for the initial state, and trivially implies the safety property.

Assume that the machine halts, and show that the invariant is inductive. The reasoning is as follows:
A state satisfying the invariant induces a partial valid tiling over the active area of the board.
%If the machine halts, this corresponds to either a partial run of the machine, or $T_{\text{halt}}$ appears on the board.
A partial valid tiling corresponds to a prefix of the machine run, so if the machine halts it must be finite, and so the active area is finite.
%If the machine halts, this corresponds to either a partial run of the machine, or $T_{\text{halt}}$ appears on the board.
%In any case the active area must be finite.
Thus, because $H$ is preserved under successor for active locations, by induction on the number of tiles in the active area, $H$ must hold for the maximal location.
Therefore, after a transition is taken, $f$ remains $\true$.
Since the transition system always places a tile that respects the horizontal and vertical constraints, and sets $H$ to true for the new maximal location, it is easy to see that the rest of the invariant is preserved by a transition as well.
%If the machine halts, a partially valid tiling corresponds to either a partial run of the machine, or $T_{\text{halt}}$ appears on the board. No tile can come after $T_{\text{halt}}$. Therefore the invariant implies that in this case the partial tiling of the board must be finite.
%Thus, by induction on the number of tiles in the active area, we can never turn $f$ to $\false$.

If the machine does not halt then there is an infinite structure encoding an infinite run. (For this we take $\text{max}$ to be an infinite oridnal of the horizontal order, to allow an infinite tape.) From this we can construct a counterexample to induction: \yotam{Neil said such a structure can be obtained from compactness, need to think about this} the transition begins with the infinite valid tiling, with an additional tile \emph{after} this infinite sequence of tiles.
(Recall that the board dimensions are axiomatized to be total orders; such a tile is placed in a location corresponding to ordinal $\omega$ of the rows order.)
This location is set to be the maximal active one.
We set $H$ to be $\false$ for this location.
Note that this does not violate the invariant: $H$ is preserved under successor of active tiles, but nonetheless does not hold for all active tiles (in essence, the induction fails).
The transition will now place a new tile and turn $f$ to $\false$.

Thus the invariant is inductive iff the Turing machine halts.
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

